Fair Densities via Boosting the Sufficient Statistics of Exponential Families

We introduce a boosting algorithm to pre-process data for fairness. Starting from an initial fair but inaccurate distribution, our approach shifts towards better data fitting while still ensuring a minimal fairness guarantee. To do so, it learns the sufficient statistics of an exponential family with boosting-compliant convergence. Importantly, we are able to theoretically prove that the learned distribution will have a representation rate and statistical rate data fairness guarantee. Unlike recent optimization based pre-processing methods, our approach can be easily adapted for continuous domain features. Furthermore, when the weak learners are specified to be decision trees, the sufficient statistics of the learned distribution can be examined to provide clues on sources of (un)fairness. Empirical results are present to display the quality of result on real-world data.

==> tables/clustering_discrete.tex <==
\begin{table*}[t]
    \caption{\fbde~(\(T = 32\)) and baselines evaluated for clustering fairness.}
    \label{tab:clustering_experiments_table}
    \begin{center}
    \begin{small}
    \begin{sc}
    \begin{tabularx}{\textwidth}{LMDDDDDDDD} %{LLMXXXXXXXX}
        \toprule
        & & Data & \mollifiera & \mollifierb & \mollifierc & \mollifierd & \celisa & \celisb & \fairkmeans \\
        \midrule
        {\multirow{3}{*}{\rotatebox[origin=c]{90}{COM.}}} 
        & $ \cPR $           &  \(.334 \pm .019\) & \(.332 \pm .022\) & \(.334 \pm .019\) & \(.334 \pm .019\) & \(.319 \pm .036\) & \(.333 \pm .020\) & \(.334 \pm .019\) & \(.259 \pm .013\) \\
        & $ \cSR $           &  \(.288 \pm .055\) & \(.235 \pm .082\) & \(.284 \pm .055\) & \(.284 \pm .055\) & \(.256 \pm .084\) & \(.288 \pm .059\) & \(.284 \pm .055\) & \(.284 \pm .036\) \\
%        & $ \cSRm $          &  \(.811 \pm .025\) & \(.820 \pm .049\) & \(.807 \pm .031\) & \(.807 \pm .031\) & \(.817 \pm .051\) & \(.804 \pm .029\) & \(.807 \pm .031\) & \(.860 \pm .038\) \\
        & $ \textrm{dist} $  &  \(.065 \pm .000\) & \(.078 \pm .000\) & \(.078 \pm .000\) & \(.078 \pm .000\) & \(.078 \pm .000\) & \(.078 \pm .000\) & \(.078 \pm .000\) & \(.069 \pm .001\) \\
        \midrule
        {\multirow{3}{*}{\rotatebox[origin=c]{90}{Adu.}}}
        & $ \cPR $           &  \(.125 \pm .067\) & \(.093 \pm .019\) & \(.101 \pm .025\) & \(.116 \pm .027\) & \(.111 \pm .033\) & \(.130 \pm .061\) & \(.097 \pm .036\) & \(.117 \pm .039\) \\
        & $ \cSR $           &  \(.426 \pm .232\) & \(.252 \pm .082\) & \(.302 \pm .076\) & \(.190 \pm .061\) & \(.254 \pm .086\) & \(.468 \pm .237\) & \(.212 \pm .129\) & \(.296 \pm .151\) \\
%        & $ \cSRm $          &  \(.421 \pm .116\) & \(.331 \pm .018\) & \(.312 \pm .035\) & \(.360 \pm .049\) & \(.346 \pm .048\) & \(.435 \pm .093\) & \(.359 \pm .045\) & \(.342 \pm .064\) \\
        & $ \textrm{dist} $  &  \(.034 \pm .000\) & \(.037 \pm .000\) & \(.037 \pm .000\) & \(.037 \pm .000\) & \(.037 \pm .000\) & \(.037 \pm .000\) & \(.037 \pm .000\) & \(.035 \pm .000\) \\
        \bottomrule
    \end{tabularx}
    \end{sc}
    \end{small}
    \end{center}
\end{table*}

==> tables/data_discrete.tex <==
\begin{table*}[t]
    \caption{\fbde~(\(T = 32\)) and baselines evaluated for data fairness and prediction fairness.}
    \label{tab:data_experiments_table}
    \begin{center}
    \begin{small}
    \begin{sc}
    \begin{tabularx}{\textwidth}{LMDDDDDDD} %{LLMXXXXXXXX}
        \toprule
        & & Data & \mollifiera & \mollifierb & \mollifierc & \mollifierd & \celisa & \celisb \\
        
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%% COMPAS %%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \midrule
        {\multirow{7}{*}{\rotatebox[origin=c]{90}{\compas}}} 
& $ \textrm{RR} $                & \(.662 \pm .007\) & \(.966 \pm .008\) & \(.977 \pm .008\) & \(.944 \pm .010\) & \(.964 \pm .009\) & \(.992 \pm .004\) & \(.990 \pm .007\) \\
& $ \textrm{SR} $                & \(.747 \pm .013\) & \(.988 \pm .006\) & \(.899 \pm .011\) & \(.978 \pm .011\) & \(.896 \pm .011\) & \(.992 \pm .006\) & \(.861 \pm .016\) \\
& $ \textrm{KL} $                & -                 & \(.135 \pm .020\) & \(.129 \pm .020\) & \(.132 \pm .020\) & \(.127 \pm .020\) & \(.164 \pm .018\) & \(.151 \pm .016\) \\
        \cmidrule(l{5pt}){2-9}
& $ \textrm{SR}_{\textrm{c}}$    & \(.747 \pm .020\) & \(.959 \pm .025\) & \(.875 \pm .025\) & \(.945 \pm .027\) & \(.872 \pm .024\) & \(.939 \pm .018\) & \(.823 \pm .017\) \\
& $ \textrm{EO} $                & \(.781 \pm .034\) & \(.960 \pm .026\) & \(.900 \pm .041\) & \(.950 \pm .028\) & \(.895 \pm .039\) & \(.944 \pm .020\) & \(.819 \pm .017\) \\
& $ \textrm{Acc} $               &
\(.660 \pm .004\) & \(.641 \pm .014\) & \(.653 \pm .012\) & \(.642 \pm .010\) & \(.656 \pm .012\) & \(.648 \pm .015\) & \(.648 \pm .015\) \\
        \midrule
        
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%  ADULT %%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        {\multirow{7}{*}{\rotatebox[origin=c]{90}{Adult}}} 
& $ \textrm{RR} $                &  \(.496 \pm .002\) & \(.958 \pm .003\) & \(.979 \pm .003\) & \(.919 \pm .004\) & \(.957 \pm .003\) & \(.995 \pm .002\) & \(.998 \pm .001\) \\
& $ \textrm{SR} $                &  \(.360 \pm .005\) & \(.961 \pm .005\) & \(.883 \pm .006\) & \(.924 \pm .006\) & \(.865 \pm .006\) & \(.979 \pm .004\) & \(.718 \pm .004\) \\
& $ \textrm{KL} $                &  -                 & \(.122 \pm .006\) & \(.119 \pm .006\) & \(.113 \pm .006\) & \(.114 \pm .006\) & \(.182 \pm .005\) & \(.164 \pm .004\) \\
        \cmidrule(l{5pt}){2-9}
& $ \textrm{SR}_{\textrm{c}}$    &  \(.360 \pm .003\) & \(.818 \pm .010\) & \(.766 \pm .010\) & \(.793 \pm .011\) & \(.753 \pm .008\) & \(.919 \pm .011\) & \(.670 \pm .008\) \\
& $ \textrm{EO} $                &  \(.471 \pm .008\) & \(.959 \pm .016\) & \(.908 \pm .018\) & \(.935 \pm .016\) & \(.895 \pm .016\) & \(.981 \pm .010\) & \(.603 \pm .015\) \\
& $ \textrm{Acc} $               &   \(.803 \pm .003\) & \(.785 \pm .002\) & \(.788 \pm .002\) & \(.787 \pm .002\) & \(.788 \pm .002\) & \(.773 \pm .005\) & \(.792 \pm .004\) \\
        \bottomrule
    \end{tabularx}
    \end{sc}
    \end{small}
    \end{center}
\end{table*}
